A Query Optimization Method Utilizing Large Language Models

Query optimization is a critical task in database systems, focused on determining the most efficient way to execute a query from an enormous set of possible strategies. Traditional approaches rely on heuristic search methods and cost predictions, but these often struggle with the complexity of the search space and inaccuracies in performance estimation, leading to suboptimal plan choices. This paper presents LLMOpt, a novel framework that leverages Large Language Models (LLMs) to address these challenges through two innovative components: (1) LLM for Plan Candidate Generation (LLMOpt(G)), which eliminates heuristic search by utilizing the reasoning abilities of LLMs to directly generate high-quality query plans, and (2) LLM for Plan Candidate Selection (LLMOpt(S)), a list-wise cost model that compares candidates globally to enhance selection accuracy. To adapt LLMs for query optimization, we propose fine-tuning pre-trained models using optimization data collected offline. Experimental results on the JOB, JOB-EXT, and Stack benchmarks show that LLMOpt(G) and LLMOpt(S) outperform state-of-the-art methods, including PostgreSQL, BAO, and HybridQO. Notably, LLMOpt(S) achieves the best practical performance, striking a balance between plan quality and inference efficiency.

==> Data_Synthesis.tex <==

\section{Data Synthesis}
\label{section:data_synthesis}

Data synthetic is a vital component while using LLMs since existing data are generated from few fixed templates with same tables and connections. As a method mainly utilizing LLMs, LLMQO has to overcome the difficulties of query synthesis. The main difficulty is to generate queries with high diversity and possible execution results as mentioned in section ~\ref{subsection:framework}. To overcome the difficulties, LLMQO utilizes GPT-4o to ensure the diversity and interacts with 
DB systems to ensure possible results. Detailed process is shown in figure ~\ref{fig:LLMQO}.

\textbf{Query Synthesis}

Firstly, we collect few queries with two or three tables as basic queries by prompting GPT-4o with database schema and few column statistics. All generated queries are executed and filtered these without execution results.

After having these queries as our base queries, we iteratively ask GPT-4o to add one more table on the given query and left the predicates on the new table to be a template (e.g. \%s). Then, we filled each template with possible value from database execution to ensure the generated query has execution results and add the query as a synthetic sql to our dataset. The filled queries are also used as base queries for the next iteration. Each iteration generates queries with more table connected and query synthesis process finally ends when there are enough queries with enough complexity. 

For example, for a query initially generated with two tables: 
\begin{equation}
    \textit{SELECT count(*) FROM mc, t WHERE mc.movie\_id = t.id;}\label{base_query}
\end{equation}
GPT-4o is asked to generate a query formed like:
\begin{equation}
\begin{split}
   \textit{SELECT count(*) FROM cn, mc, t WHERE cn.country\_code =}\\
    \textit{\%s AND cn.id = mc.company\_id AND mc.movie\_id = t.id;} \label{template_query}
\end{split}
 \end{equation}
 
, in which a new table cn is connected with existed table mc and the predicate \textit{cn.country\_code = \%s} is a template formulation. The filled value \%s has to ensure there are execution results for the complete query. Therefore, based on query ~\ref{template_query}, we select the possible values of \%s by executing the following query:
\begin{equation}
\begin{split}
   \textit{SELECT cn.country\_code FROM cn, mc, t WHERE}\\
    \textit{ cn.id = mc.company\_id AND mc.movie\_id = t.id;} \label{value_query}
\end{split}
 \end{equation}

It is noticing that query ~\ref{value_query} may have no results or syntax error due to the fact that the new table \textit{cn} and the connection \textit{cn.id = mc.company\_id} 
are generated from GPT-4o. Therefore, database schema are given to GPT-4o to avoid syntax error. 

We sample few results of query ~\ref{value_query} (e.g. '[de]') and finally filled the template query ~\ref{template_query}:
\begin{equation}
\begin{split}
   \textit{SELECT count(*) FROM cn, mc, t WHERE cn.country\_code =}\\
    \textit{'[de]' AND cn.id = mc.company\_id AND mc.movie\_id = t.id;} \label{filled_query}
\end{split}
 \end{equation}

Each result of query ~\ref{value_query} can be filled into the template query ~\ref{template_query}. Therefore, we can generate several similar queries with different results to enhance the generalize ability of LLMs. Furthermore, the queries are more diverse after several iterations. In conclusion, we synthesis multiple queries with high diversity and explicit execution results by iteratively prompting GPT-4o and retrieve values from DB systems.


\textbf{Label Collection}
To implement query optimization tasks with fine-tuned LLMs, we need to collect labels for each query as training data. This means we need to find an optimal plan for each sql. As mentioned in Bao\cite{marcus2021bao}, 5 $Bao\_arms$ leads to 93\% of the improvements, which inspires us of using these arms to collect labels. We suppose that the optimal plan is among those candidates and execute every one to obtain the latency. Therefore, we are able to choose the optimal one and its corresponding hints $h^*$ as the label in training generative model and selective model. 



==> intro.tex <==
\section{Introduction}

In modern corporations, a huge amount of queries are executed in databases for daily businesses. 
Query Optimization as an important task in database aims to accelerate query execution. In order to execute query in an efficient way, query plans are searched in a massive plan space with $O(n!)$ complexity where $n$ denotes to the number of tables in the given query. 
In database management systems (DBMS) such as PostgreSQL (PG), a dynamic programming algorithm is designed to search for an optimal query plan by iteratively connecting new table to an existing sub-plan and pruning those with estimated poor performances. Due to the incorrect estimation of conventional optimizer, researchers have proposed multiple methods\cite{marcus2021bao,chen2023leon,marcus2019neo,yang2022balsa,zhu2023lero} with machine-learning models aided to replace or enhance the conventional optimizer. Generally, all methods follows a searching-selecting pipeline shown in figure \ref{fig:pipeline}. However, there is a main limitation for this pipeline.


% For a query with $n$ tables connected, there are $O(n!)$ physical query plans in the search space maintaining different join orders, join types and scan types. The numerous search space implies the problem as NP-hard. Therefore, modern database management systems (DBMS) implement a dynamic programming algorithm. For example, PostgreSQL (PG) iteratively generates sub-plans from a single table to a full query plan and utilizes a heuristic cost model to select the best sub-plan in each iteration. However, the inaccuracy of cost model fails to generate an optimized plan. 
%To improve the performance of query optimizer, there are two main approaches proposed.


% To improve the performance of query optimizer, multiple methods\cite{marcus2021bao, } are proposed to enhance or replace the traditional optimizer, following a pipeline shown in figure \ref{fig:pipeline}. Generally, the pipeline separate query optimization 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/Example.png}
    \caption{Limitations of Existing Methods}
    \label{fig:example}
\end{figure}


\vpara{Massive Searching Space.} Heuristic searching algorithm in existing methods limits the possibility of finding optimal plan in candidate set. For a query with $n$ tables, there are a massive searching space with $O(n!)$ query plans. Firstly, the numbers of different tree structures follows Catalan number which has a complexity of $O(n!)$ \cite{stanley2015catalan}. For example, as shown in figure \ref{fig:example} (a), a query with 5 tables derives 14 different tree structures. Secondly, to fill leaf nodes in the planning tree with tables, there are multiple sequences. Lastly, there are several node types representing physical executing operators for scan and join nodes. Conventional methods use dynamic algorithm to search for optimal plan and utilize a cost model to prune searching process, which is limited to the accuracy of cost model and leads to sub-optimal plan.
At the same time, existing methods such as Bao\cite{marcus2021bao} and QueryFormer\cite{zhao2022queryformer} modify conventional optimizer which may be unable to find an optimal plan in a candidate set. 

% \vpara{(2) Poor Selecting Result.} Cost models with a structure of tree convolution neural networks (Tree-CNN) in Bao\cite{marcus2021bao} or tree-LSTM in HybridQO\cite{yu2022cost} sometimes fail to selecting an optimal plan as shown in figure \ref{fig:example} (b). The optimal shown in figure \ref{fig:example} (b) is the optimal plan in candidate set. For example, for query 18c in join-order-benchmark (JOB), Bao fails to select the optimal one, leaving a 20\% optimization space. And for query 17b, Bao has a worse performance than PG while the optimal plan yields a approximately 50\% improvement. Moreover, recent works\cite{lehmann2023your,zhao2023comparative} have proved that existing methods failed to outperform PG in end-to-end latency. 
% Therefore, we doubt the ability of existing cost models with a small amount of parameters.

Due to the limitation mentioned above, large language models (LLMs) seems to be a possible solution. 
Recent LLMs such as GPT-4\cite{openai2023gpt4} and DeepSeek-v3\cite{liu2024deepseek} has exhibited powerful natural language generating and understanding abilities. 
Firstly, LLMs can straightly generate textual contents for tasks such as QA\cite{li2022self}. While natural language has a larger searching space than query optimization tasks, LLMs are able to generate reasonable outputs for users, indicating its powerful generating ability. In query optimization, LLMs may be helpful to generate optimal plan from the massive searching space. 
Secondly, LLMs has powerful understanding and reasoning abilities\cite{hurst2024gpt,guo2025deepseek}, especially in coding\cite{chew2023llm,jiang2024survey} and math\cite{imani2023mathprompter} tasks. Query optimization tasks also requires high reasoning ability of utilizing rules to search an optimal plan.
Moreover, in-context-learning\cite{shin2022effect} is also a important ability of LLM which enables it to enhance the result from external knowledge given by prompt. In query optimization, each query has relevant metrics which are helpful for optimizers and can be used as external knowledge for LLM. 

Recently, LLMs are proven useful in database domain. Researchers have explored the usage of LLMs in text-to-sql\cite{dong2023c3,li2024codes}, knob tuning\cite{huang2024llmtune,giannakouris2024demonstrating} and query rewrite\cite{ma2023query,liu2024query}. Therefore, we suppose LLMs useful in query optimization as well. 

% In textual tasks such as coding\cite{jiang2024survey,xu2022systematic}, and QA\cite{chang2024survey}, LLMs are able to follow instructions and generating reasonable answers to specific tasks. 

% \vpara{(1) Powerful Generating Ability.} 
% LLM has powerful generation ability which can straightly generate an optimal plan from the massive searching space rather than using a dynamic programming algorithm. The model structure for LLM enables it to efficiently generate textual content with amazing effect. GPT-4\cite{openai2023gpt4} and Deepseek-V3\cite{liu2024deepseek} has shown the powerful generating ability in textual tasks. This inspires us to utilize LLM for query optimization since query plans can be easily represented to a textual content. Therefore, we replace the candidate searching with a LLM which are more likely to generate an optimal plan.

% \vpara{(2) High Understanding Ability.} 
% With a numerous amount of parameters, LLMs have high understanding ability. With supervised fine-tuning, we are able to 

To utilize LLM in query optimization, there are some preparations. Firstly, we need to serialize query plans to textual content as output of LLM. Secondly, the external knowledge is also important for LLMs. While these preparations are done as demonstrated in section \ref{subsection:pg_hint_plan} and section \ref{section:data_collection}, we propose \Model, a \textbf{L}arge \textbf{Lan}guage \textbf{M}odel \textbf{O}ptimizer which investigates potential approaches for utilizing LLMs as query optimizers. The framework of \Model is shown in figure \ref{fig:pipeline}.

\vpara{LLM for Plan Generation.} A obvious method of utilizing LLMs is an end-to-end approach. With a given query, LLM straightforwardly generate an optimal query plan. However, it is hard for pre-trained LLMs(PLMs) such as Llama-3.1\cite{dubey2024llama} to complete query optimization tasks although these models reaches high score in natural language tasks. This is because PLMs haven't been seen inputs and outputs of query optimization task and are unable to comprehend the task to generate valid outputs. Therefore, we supervised fine-tune a PLM with pre-collected data offline for query optimization. 

However, this approach are limited to high inference cost. While machine-learning models are powerful in improving query plans\cite{marcus2021bao,zhu2023lero,chen2023leon}, these methods waste a lot of time in inference and lead to worse performance than PG\cite{lehmann2023your}. LLM spend more time on inference due to its transformers structure and numerous parameters. Concerning the inference cost, we propose another approach.

\vpara{LLM for Plan Selection.} Noticing existing searching-selecting pipeline, another approach is to utilize LLM for plan selection. While other ML-aided methods train a point-wise or pair-wise cost model which requires multiple inferences for each query, LLMs have the potential to be a list-wise cost model. This reduces the inference cost 

% \vpara{(1) Unable to comprehend query optimization.} Although open source LLMs such as LlaMA-3.1\cite{dubey2024llama} are powerful in natural language tasks, it is hard for LLMs to comprehend query optimization tasks since these models haven't been trained on query optimization dataset before. Even after supervised fine-tuning, there are still possibilities for LLM to generate invalid output with wrong format or poor performances. 

% \vpara{(2) High inference cost.} While machine-learning models are powerful in improving query plans\cite{marcus2021bao,zhu2023lero,chen2023leon}, these methods waste a lot of time in inference and lead to worse performance than PG\cite{lehmann2023your}. LLM faces more difficulties as its numerous parameters require more time to inference for a complete query plan. 

% Addition to these challenges, we propose \Model, a \textbf{L}arge \textbf{Lan}guage \textbf{M}odel \textbf{O}ptimizer which investigates two potential approaches for utilizing LLMs as query optimizers. The core idea of \Model is to utilize large language models (LLMs) and overcome difficulties encountered in previous methods. The framework of \Model is shown in figure \ref{fig:pipeline}. 

% To excavate the generation ability of LLM, the first approach in \Model is to replace candidate searching with a LLM as generative model. Rather than generating one plan for each query, we sample LLM to generate multiple plans as candidates, which gives a fault tolerance for invalid format or poor performance. We use Tree-CNN as cost model to select optimal query plan from candidate plans.

% Then, to reduce inference cost, another approach replace the cost model in pipeline with a supervised fine-tuned LLM as selective model. With the usage as a list-wise cost model, LLM is able to infer once per query and generate one token representing the optimal plan per inference to fulfill this task. In LLM's basic transformer structure, this reduce a lot of time compared to generating a complete query plan. 




% In query optimization task, this enables us to use LLM to select an optimal plan among candidate set. With the idea of generating as less tokens as possible to reduce inference cost, we propose another approach with the replacement of cost models in candidate selection. Due to the high understanding ability, \Model not only improve the execution latency of the selected plan, but improve the end-to-end latency as well. 

Our experimental result shown that the selective model in \Model outperforms existing methods in execution latency and end-to-end latency. At the same time, the generative model in \Model also provides better query plans than existing methods. Our detailed evaluation on generative model and selective model also proves the powerful capability of LLMs in query optimization. 

% Addition to problems mentioned above, we propose LLMQO (Large Language Model Query Optimization), the first method utilizing large language models in query optimization task.
% While generative large language models (LLMs) such as GPT-4\cite{} and Llama-3\cite{} are proved to be powerful in generation tasks, we suppose it may help in query optimization by replacing both components in the pipeline. The language ability enlarges the search space in candidate generation which means we are more likely to find an optimal plan in our candidates. Details of our generative model are discussed in section \ref{}.
% The large scale of parameters also enables LLMs to act as a powerful cost model and select an optimal plan from candidates. This part is shown in section \ref{}. To explore the zero-shot ability and few-shot ability of LLMs, we synthesis large amount of traning data with high diversity, which are discussed in section \ref{}.


% Generally, existing methods are summarized into two approaches. The first approach follows the traditional algorithm used by PG and replaces the heuristic cost model with a machine learning model. Neo\cite{}, LEON\cite{} and Balsa\cite{} are typical methods from this approach. The second approach generates various query plans by adding constraints to DBMS and trains a machine learning model to select the optimal plan. Bao\cite{marcus2021bao}, QueryFormer\cite{} and HyperQO\cite{} follow this approach.
% Details of each approach are discussed in section \ref{subsection:pipeline}. It is noticing that both approach has two components: candidate generation and candidate selection. However, there are several limitations in existing methods.

% \textbf{(1) Limited Search Spaces.} Existing methods mainly focus on candidate selection and ignores the various search spaces of plans. Bao\cite{marcus2021bao} and some other methods\cite{} uses some database knobs to restrict the traditional optimizer and generate different plans. Due to its wide influence on other query optimization methods and our work, we discuss Bao later in section \ref{}. HyperQO\cite{} uses Monte-Carlo Tree Search (MCTS) to generate possible table connecting orders for a plugin \textit{pg\_hint\_plan} to generate candidate plans. Details of \textit{pg\_hint\_plan} are discussed in section \ref{}.
% However, all methods mentioned above use heuristic methods to generate candidates and are limited to the traditional methods since the candidates are finally generated by DBMS. Therefore, the optimal plan may not be taken into consideration which leads to poor performance. 

% \textbf{(2) Poor ability of Cost Models.} Cost model as the guideline of candidate selection, is the core of existing methods. Different from conventional methods using rule-based cost models in DBMS, modern methods build various machine learning structures. Neo\cite{}, Bao\cite{marcus2021bao} and some methods use tree convolution neural networks(TCNN) to encode query features and plan features and predict the performance of a single query. RTOS\cite{}, LOGER\cite{} and HyperQO\cite{} uses tree-structured LSTM(Tree-LSTM) to encode the plan tree. However, features given for the cost models varies in different methods. While little scaled models are unable to develop the rules to predict the latency with all related features, it is also hard to select an optimal plan with limited information. At the same time, recent studies\cite{} find that inference time highly hack in end-to-end time since the improvement of execution latency are smoothed out by inference time, especially in methods following the first approach since the extensively usage of cost model. 

% \textbf{(3) Requirement for Data with Same Templates.} Existing methods has poor zero-shot and few-shot abilities due to the model structure and limited training data. Training data used for existing methods has high similarity, with same tables connected and same selections and little predicates shift. Therefore, for an unseen workload, existing methods failed to generalize on it to achieve a well performance. 

%The first approach uses learn-based cost model to replace the heuristic cost model in dynamic programming algorithm. This approach maintains the framework of traditional optimizer and changes the model to a machine learning one. In each iteration, a local cost model is used to predict the best sub-plan with same joined tables. After each iteration, a global cost model is used to prune sub-plans with different joined tables.  
%The second approach keeps database system stabled and generates different candidate query plans for a machine learning cost model to predict the execution latency and select the best one with the lowest latency to execute. 
% However, there are some drawbacks for both approaches:

% (1)\textbf{Limited Search Spaces.} For the first approach, the pruning action reducing search space is a double-edged sword. The selection of sub-optimal plan in each iteration may lead to poor generated query plan. On the other hand, the second approach uses heuristic method to generate candidate query plans, which limits the capability of generating optimal plan.

% (2)\textbf{Poor Generalization to New Databases.} All approaches differs on cost model networks and encoded features. However, the features are highly correlated with database schema. For each database, previous methods requires a large amount of data for re-training to reach a well performance. 


%一些实验相关的内容，最后来写
% To experimentally 

% For each given query, LLMQO mainly utilizes a large language model (LLM) to generate a query plan and implements it by a modified PG plugin, pg\_hint\_plan. Different from cost models, LLM straightly generate a query plan with hints used by pg\_hint\_plan rather than giving an order or cost estimation of a list of candidate plans. Since it is a generative model, it has a larger search space and a higher possibility to reach the "best" plan. Previous works on LLMs \cite{} have proven that LLMs are capable to generalize on workload shift. So we suppose it can learn the methodology of queries and data distributions in different database schema and it is verified by our experimental results. However, while utilizing LLMs, there are some challenges:

% (1) \textbf{Lack of Training Data}. Due to LLM's encoding structure, it requires enough data diversity, which are not fully demonstrated in previous works. Recent studies \cite{} uses OLAP benchmarks and extends queries as training data. However, most of the training data are generated from same template, which means these have independent and identically distribution. Furthermore, there are an overall hypothesis on query optimization tasks, which is the query have at least one executed result. It is noticing that the earlier a sub-plan with no result is executed, the faster the query is, since there is no need to execute other table scan or join. However, it is nearly impossible to predict which of the table scan turns out to be no result. Therefore, all of the queries should have at least one result to ensure all of the sub-queries have results. To efficiently synthetic queries with valid results, we propose a method prompting GPT-4o to generate templates and filling template by extracting values from databases. 

%这部分可能不讲了
%(2)\textbf{}  Since there are numerous language spaces for LLMs, we may have chaotic and meaningless outputs. Although pre-training may help LLMs to avoid these shortcomings, there are still possibilities for LLMs to give a result unable to reconstruct a query plan. Therefore, inspired by previous works on cost model, we propose two different types of LLM: one is to select the best query plan from a given plan lists and act as a cost model, and another one is to generate the predicted best query plan with a larger searching space. With two different modes, our LLM has both exploration and exploitation. 

% 是否要讲drawbacks...
% There are some drawbacks of LLMQO since the usage of LLMs. A significant drawback is that LLMQO requires enough device to deploy a LLM, which is not common in database systems. Another drawback is that LLM inference spend more time that other ML methods and conventional methods in database systems due to its large scale of parameters. Recent works \cite{} has shown that most query optimization failed to overcome PG because of a high inference latency. We believe works on LLMs will improve inference efficiency and this will not be a problem in future. Therefore, we only focus on the execution latency of each query.

Our main contributions are summarized:
\begin{itemize}
    \item We firstly proposed a query optimization method utilizing large language models(LLMs) to generate an optimal query plan with larger searching space rather than searching a query plan from the massive searching space. The usage of LLMs highly improves the possibility to generate an optimal plan.
    \item Our usage of LLMs in candidate selection improves the end-to-end performance in query optimization while utilizing LLMs often spend a lot of time in inference. 
    
    \item Our experimental result proves that \Model outperforms all existing open-source query optimization methods and simply prompting well-known LLMs such as GPT-4. LLMs shown capability to understand the differences between candidate query plans and generate a better one.
    % , which enables LLMQO to enhance itself.
\end{itemize}

==> tables/end2end.tex <==
\begin{table}[t]
\centering
\caption{End-to-end latency (s)$\downarrow$ of \Model and other baselines.}
\label{tab:end2end}
\begin{tabular}{cccc}
\toprule
 & JOB\cite{Job} & JOB-EXT\cite{marcus2019neo} & Stack\cite{marcus2021bao} \\
\midrule
PostgreSQL & 129.34& 66.55 & \underline{335.62} \\
BAO\cite{marcus2021bao} & \underline{75.88}& 62.72 &  410.38\\
HybridQO\cite{yu2022cost} &183.87& 84.62  & 1097.73 \\
\Model (G) & 148.78 & \textbf{55.98} &385.07 \\
\Model (S) & \textbf{62.51} & \underline{61.07}  & \textbf{236.15}
 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/maximal_potential.tex <==
\begin{table}[htbp]
\centering
\caption{Execution latencies (s) $\downarrow$ of workloads with optimal plan.}
\label{tab:generative_optimal}
\begin{tabular}{cccc}
\toprule
 & JOB\cite{Job} &JOB-EXT\cite{marcus2019neo}& Stack\cite{marcus2021bao} \\
\midrule
PG & 129.26& 66.41 & 334.66 \\
\Baoarm s\cite{marcus2021bao} & 35.62& 49.46 &  210.92 \\
MCTS \cite{yu2022cost} & 96.46 & 55.53& 332.58\\
$LLM^G$ & \textbf{33.74} & \textbf{45.09}
 & \textbf{202.88}
 \\
\bottomrule
\end{tabular}
\end{table}

==> training_cost.tex <==
\section{Training Cost}
